ConvNets and ImageNet Beyond Accuracy: Understanding Mistakes and Uncovering Biases

ConvNets and Imagenet have driven the recent success of deep learning for image classification. However, the marked slowdown in performance improvement combined with the lack of robustness of neural networks to adversarial examples and their tendency to exhibit undesirable biases question the reliability of these methods. This work investigates these questions from the perspective of the end-user by using human subject studies and explanations. The contribution of this study is threefold. We first experimentally demonstrate that the accuracy and robustness of ConvNets measured on Imagenet are vastly underestimated. Next, we show that explanations can mitigate the impact of misclassified adversarial examples from the perspective of the end-user. We finally introduce a novel tool for uncovering the undesirable biases learned by a model. These contributions also show that explanations are a valuable tool both for improving our understanding of ConvNets' predictions and for designing more reliable models.

==> arxiv copy/definitions.tex <==
\usepackage{graphicx} % more modern
%\usepackage{epsfig} % less modern
%\usepackage[round,authoryear,sort]{natbib}
\usepackage{amsmath,amsthm,amssymb,bbm,stmaryrd,bm}
%\usepackage{url}

\usepackage{dsfont}
\usepackage{color}
\usepackage{wrapfig}
\usepackage{listing}
\usepackage{amsopn}
%\usepackage[breaklinks=true]{hyperref}

\newcommand{\todo}[1]{{\color{red}{To do: #1}}}

% %%%%%%%%%%%%%  VECTORS %%%%%%%%%%%%%%%%%%%
\newcommand{\bmt}[1]{\bm{#1}^T} % transpose of a vector
% INNER PRODUCT <x,y>
\newcommand{\ip}[2]{\langle {#1},\, {#2} x`\rangle}

% \va, \vb etc. type bold letters; notice exception at \vech -- coz. \vh is a
% predefined thing in latex; 
% additional commands include \vah -- read as vector a hat, 
% or \ah -- a hat and so on
\newcommand{\va}{\bm{a}}       \newcommand{\vah}{\hat{\bm{a}}}        \newcommand{\ah}{\hat{a}}
\newcommand{\vb}{\bm{b}}       \newcommand{\vbh}{\hat{\bm{b}}}        \newcommand{\bh}{\hat{b}}
\newcommand{\vc}{\bm{c}}       \newcommand{\vch}{\hat{\bm{c}}}        \newcommand{\ch}{\hat{c}}
\newcommand{\vd}{\bm{d}}       \newcommand{\vdh}{\hat{\bm{d}}}        \newcommand{\dhat}{\hat{d}}
\newcommand{\ve}{\bm{e}}       \newcommand{\veh}{\hat{\bm{e}}}        \newcommand{\eh}{\hat{e}}
\newcommand{\vf}{\bm{f}}       \newcommand{\vfh}{\hat{\bm{f}}}        \newcommand{\fh}{\hat{f}}
\newcommand{\vg}{\bm{g}}       \newcommand{\vgh}{\hat{\bm{g}}}        \newcommand{\gh}{\hat{g}}
\newcommand{\vech}{\bm{h}}     \newcommand{\vhh}{\hat{\bm{h}}}        \newcommand{\hh}{\hat{h}}
\newcommand{\vi}{\bm{i}}       \newcommand{\vih}{\hat{\bm{i}}}        \newcommand{\ih}{\hat{i}}
\newcommand{\vj}{\bm{j}}       \newcommand{\vjh}{\hat{\bm{j}}}        \newcommand{\jh}{\hat{j}}
\newcommand{\vk}{\bm{k}}       \newcommand{\vkh}{\hat{\bm{k}}}        \newcommand{\kh}{\hat{k}}
\newcommand{\vl}{\bm{l}}       \newcommand{\vlh}{\hat{\bm{l}}}        \newcommand{\lh}{\hat{l}}
\newcommand{\vm}{\bm{m}}       \newcommand{\vmh}{\hat{\bm{m}}}        \newcommand{\mh}{\hat{m}}
\newcommand{\vn}{\bm{n}}       \newcommand{\vnh}{\hat{\bm{n}}}        \newcommand{\nh}{\hat{n}}
\newcommand{\vo}{\bm{o}}       \newcommand{\voh}{\hat{\bm{o}}}        \newcommand{\oh}{\hat{o}}
\newcommand{\vp}{\bm{p}}       \newcommand{\vph}{\hat{\bm{p}}}        \newcommand{\ph}{\hat{p}}
\newcommand{\vq}{\bm{q}}       \newcommand{\vqh}{\hat{\bm{q}}}        \newcommand{\qh}{\hat{q}}
\newcommand{\vr}{\bm{r}}       \newcommand{\vrh}{\hat{\bm{r}}}        \newcommand{\rh}{\hat{r}}
\newcommand{\vs}{\bm{s}}       \newcommand{\vsh}{\hat{\bm{s}}}        \newcommand{\sh}{\hat{s}}
\newcommand{\vt}{\bm{t}}       \newcommand{\vth}{\hat{\bm{t}}}        \newcommand{\that}{\hat{t}}
\newcommand{\vu}{\bm{u}}       \newcommand{\vuh}{\hat{\bm{u}}}        \newcommand{\uh}{\hat{u}}
\newcommand{\vv}{\bm{v}}       \newcommand{\vvh}{\hat{\bm{v}}}        \newcommand{\vh}{\hat{v}}
\newcommand{\vw}{\bm{w}}       \newcommand{\vwh}{\hat{\bm{w}}}        \newcommand{\wh}{\hat{w}}
\newcommand{\vx}{\bm{x}}       \newcommand{\vxh}{\hat{\bm{x}}}        \newcommand{\xh}{\hat{x}}
\newcommand{\vy}{\bm{y}}       \newcommand{\vyh}{\hat{\bm{y}}}        \newcommand{\yh}{\hat{y}}
\newcommand{\vz}{\bm{z}}       \newcommand{\vzh}{\hat{\bm{z}}}        \newcommand{\zh}{\hat{z}}

% %%%%%%%%%%%%%%%%%%%% BOLD GREEK %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Same convention as for ordinary roman letters above
\newcommand{\valpha}  {\bm{\alpha}}      \newcommand{\valphah}  {\hat{\bm{\alpha}}}   
\newcommand{\vbeta}   {\bm{\beta}}       \newcommand{\vbetah}   {\hat{\bm{\beta}}}    
\newcommand{\vdelta}  {\bm{\delta}}      \newcommand{\vdeltah}  {\hat{\bm{\delta}}}   
\newcommand{\vepsilon}{\bm{\epsilon}}    \newcommand{\vepsilonh}{\hat{\bm{\epsilon}}} 
\newcommand{\vphi}    {\bm{\phi}}        \newcommand{\vphih}    {\hat{\bm{\phi}}}     
\newcommand{\vgamma}  {\bm{\gamma}}      \newcommand{\vgammah}  {\hat{\bm{\gamma}}}   
\newcommand{\veta}    {\bm{\eta}}        \newcommand{\vetah}    {\hat{\bm{\eta}}}     
\newcommand{\vtheta}  {\bm{\theta}}      \newcommand{\vthetah}  {\hat{\bm{\theta}}}   
\newcommand{\vkappa}  {\bm{\kappa}}      \newcommand{\vkappah}  {\hat{\bm{\kappa}}}   
\newcommand{\vlambda} {\bm{\lambda}}     \newcommand{\vlambdah} {\hat{\bm{\lambda}}}  
\newcommand{\vmu}     {\bm{\mu}}         \newcommand{\vmuh}     {\hat{\bm{\mu}}}      
\newcommand{\vnu}     {\bm{\nu}}         \newcommand{\vnuh}     {\hat{\bm{\nu}}}      
\newcommand{\vpi}     {\bm{\pi}}         \newcommand{\vpih}     {\hat{\bm{\pi}}}      
\newcommand{\vchi}    {\bm{\chi}}        \newcommand{\vchih}    {\hat{\bm{\chi}}}     
\newcommand{\vrho}    {\bm{\rho}}        \newcommand{\vrhoh}    {\hat{\bm{\rho}}}     
\newcommand{\vsigma}  {\bm{\sigma}}      \newcommand{\vsigmah}  {\hat{\bm{\sigma}}}   
\newcommand{\vtau}    {\bm{\tau}}        \newcommand{\vtauh}    {\hat{\bm{\tau}}}     
\newcommand{\vupsilon}{\bm{\upsilon}}    \newcommand{\vupsilonh}{\hat{\bm{\upsilon}}} 
\newcommand{\vomega}  {\bm{\omega}}      \newcommand{\vomegah}  {\hat{\bm{\omega}}}   
\newcommand{\vxi}     {\bm{\xi}}         \newcommand{\vxih}     {\hat{\bm{\xi}}}      
\newcommand{\vpsi}    {\bm{\psi}}        \newcommand{\vpsih}    {\hat{\bm{\psi}}}     
\newcommand{\vzeta}   {\bm{\zeta}}       \newcommand{\vzetah}   {\hat{\bm{\zeta}}}

% %%%%%%%%%%%%%  MATRICES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\newcommand{\ma}{\bm{A}}       \newcommand{\mah}{\hat{\bm{A}}}   
\newcommand{\mb}{\bm{B}}       \newcommand{\mbh}{\hat{\bm{B}}}   
\newcommand{\mc}{\bm{C}}       \newcommand{\mch}{\hat{\bm{C}}}   
\newcommand{\md}{\bm{D}}       \newcommand{\mdh}{\hat{\bm{D}}}   
\newcommand{\me}{\bm{E}}       \newcommand{\meh}{\hat{\bm{E}}}   
\newcommand{\mf}{\bm{F}}       \newcommand{\mfh}{\hat{\bm{F}}}   
\newcommand{\mg}{\bm{G}}       \newcommand{\mgh}{\hat{\bm{G}}}   
\newcommand{\mH}{\bm{H}}       \newcommand{\mhh}{\hat{\bm{H}}}   
\newcommand{\mi}{\bm{I}}       \newcommand{\mih}{\hat{\bm{I}}}   
\newcommand{\mj}{\bm{J}}       \newcommand{\mjh}{\hat{\bm{J}}}   
\newcommand{\mk}{\bm{K}}       \newcommand{\mkh}{\hat{\bm{K}}}   
\newcommand{\ml}{\bm{L}}       \newcommand{\mlh}{\hat{\bm{L}}}   
\newcommand{\mm}{\bm{M}}       \newcommand{\mmh}{\hat{\bm{M}}}   
\newcommand{\mn}{\bm{N}}       \newcommand{\mnh}{\hat{\bm{N}}}   
\newcommand{\mo}{\bm{O}}       \newcommand{\moh}{\hat{\bm{O}}}   
\newcommand{\mP}{\bm{P}}       \newcommand{\mph}{\hat{\bm{P}}}   
\newcommand{\mq}{\bm{Q}}       \newcommand{\mqh}{\hat{\bm{Q}}}   
\newcommand{\mr}{\bm{R}}       \newcommand{\mrh}{\hat{\bm{R}}}   
\newcommand{\ms}{\bm{S}}       \newcommand{\msh}{\hat{\bm{S}}}   
\newcommand{\mT}{\bm{T}}       \newcommand{\mth}{\hat{\bm{T}}}   
\newcommand{\mU}{\bm{U}}       \newcommand{\muh}{\hat{\bm{U}}}   
\newcommand{\mv}{\bm{V}}       \newcommand{\mvh}{\hat{\bm{V}}}   
\newcommand{\mw}{\bm{W}}       \newcommand{\mwh}{\hat{\bm{W}}}   
\newcommand{\mx}{\bm{X}}       \newcommand{\mxh}{\hat{\bm{X}}}   
\newcommand{\my}{\bm{Y}}       \newcommand{\myh}{\hat{\bm{Y}}}   
\newcommand{\mz}{\bm{Z}}       \newcommand{\mzh}{\hat{\bm{Z}}}   

%%%%%%%%%%%%%%%%%%%%%%%%% CALLIGRAPHIC LETTERS %%%%%%%%%%%%%%%%%%%%%
\newcommand{\ac}{\mathcal{a}}    \newcommand{\Ac}{\mathcal{A}}  
\newcommand{\bc}{\mathcal{b}}    \newcommand{\Bc}{\mathcal{B}}  
\newcommand{\cc}{\mathcal{c}}    \newcommand{\Cc}{\mathcal{C}}  
\newcommand{\dc}{\mathcal{d}}    \newcommand{\Dc}{\mathcal{D}}  
\newcommand{\ec}{\mathcal{e}}    \newcommand{\Ec}{\mathcal{E}}  
\newcommand{\fc}{\mathcal{f}}    \newcommand{\Fc}{\mathcal{F}}  
\newcommand{\gc}{\mathcal{g}}    \newcommand{\Gc}{\mathcal{G}}  
\newcommand{\hc}{\mathcal{h}}    \newcommand{\Hc}{\mathcal{H}}  
\newcommand{\ic}{\mathcal{i}}    \newcommand{\Ic}{\mathcal{I}}  
\newcommand{\jc}{\mathcal{j}}    \newcommand{\Jc}{\mathcal{J}}  
\newcommand{\kc}{\mathcal{k}}    \newcommand{\Kc}{\mathcal{K}}  
\newcommand{\lc}{\mathcal{l}}    \newcommand{\Lc}{\mathcal{L}}  
\newcommand{\mcal}{\mathcal{m}}  \newcommand{\Mc}{\mathcal{M}}  
\newcommand{\nc}{\mathcal{n}}    \newcommand{\Nc}{\mathcal{N}}  
\newcommand{\oc}{\mathcal{o}}    \newcommand{\Oc}{\mathcal{O}}  
\newcommand{\pc}{\mathcal{p}}    \newcommand{\Pc}{\mathcal{P}}  
\newcommand{\qc}{\mathcal{q}}    \newcommand{\Qc}{\mathcal{Q}}  
\newcommand{\rc}{\mathcal{r}}    \newcommand{\Rc}{\mathcal{R}}  
\newcommand{\scal}{\mathcal{s}}  \newcommand{\Sc}{\mathcal{S}}  
\newcommand{\tc}{\mathcal{t}}    \newcommand{\Tc}{\mathcal{T}}  
\newcommand{\uc}{\mathcal{u}}    \newcommand{\Uc}{\mathcal{U}}  
\newcommand{\vcal}{\mathcal{v}}  \newcommand{\Vc}{\mathcal{V}}  
\newcommand{\wc}{\mathcal{w}}    \newcommand{\Wc}{\mathcal{W}}  
\newcommand{\xc}{\mathcal{x}}    \newcommand{\Xc}{\mathcal{X}}  
\newcommand{\yc}{\mathcal{y}}    \newcommand{\Yc}{\mathcal{Y}}  
\newcommand{\zc}{\mathcal{z}}    \newcommand{\Zc}{\mathcal{Z}}  

%%%%%%%%%%%%%%%%%%%%%%%%% MATHEMATIC LETTERS %%%%%%%%%%%%%%%%%%%%%
\newcommand{\ar}{\mathrm{a}}    \newcommand{\Ars}{\mathrm{A}}  
\newcommand{\br}{\mathrm{b}}    \newcommand{\Br}{\mathrm{B}}  
\newcommand{\crm}{\mathrm{c}}    \newcommand{\Cr}{\mathrm{C}}  
\newcommand{\dr}{\mathrm{d}}    \newcommand{\Dr}{\mathrm{D}}  
\newcommand{\er}{\mathrm{e}}    \newcommand{\Er}{\mathrm{E}}  
\newcommand{\fr}{\mathrm{f}}    \newcommand{\Fr}{\mathrm{F}}  
\newcommand{\gr}{\mathrm{g}}    \newcommand{\Gr}{\mathrm{G}}  
\newcommand{\hr}{\mathrm{h}}    \newcommand{\Hr}{\mathrm{H}}  
\newcommand{\ir}{\mathrm{i}}    \newcommand{\Ir}{\mathrm{I}}  
\newcommand{\jr}{\mathrm{j}}    \newcommand{\Jr}{\mathrm{J}}  
\newcommand{\kr}{\mathrm{k}}    \newcommand{\Kr}{\mathrm{K}}  
\newcommand{\lr}{\mathrm{l}}    \newcommand{\Lr}{\mathrm{L}}  
\newcommand{\mrml}{\mathrm{m}}  \newcommand{\Mr}{\mathrm{M}}  
\newcommand{\nr}{\mathrm{n}}    \newcommand{\Nr}{\mathrm{N}}  
\newcommand{\orm}{\mathrm{o}}    \newcommand{\Orm}{\mathrm{O}}  
\newcommand{\pr}{\mathrm{p}}    \newcommand{\Prm}{\mathrm{P}}  
\newcommand{\qr}{\mathrm{q}}    \newcommand{\Qr}{\mathrm{Q}}  
\newcommand{\rr}{\mathrm{r}}    \newcommand{\Rr}{\mathrm{R}}  
\newcommand{\srm}{\mathrm{s}}  \newcommand{\Sr}{\mathrm{S}}  
\newcommand{\tr}{\mathrm{t}}    \newcommand{\Tr}{\mathrm{T}}  
\newcommand{\ur}{\mathrm{u}}    \newcommand{\Ur}{\mathrm{U}}  
\newcommand{\vrm}{\mathrm{v}}  \newcommand{\Vr}{\mathrm{V}}  
\newcommand{\wrm}{\mathrm{w}}    \newcommand{\Wr}{\mathrm{W}}  
\newcommand{\xr}{\mathrm{x}}    \newcommand{\Xr}{\mathrm{X}}  
\newcommand{\yr}{\mathrm{y}}    \newcommand{\Yr}{\mathrm{Y}}  
\newcommand{\zr}{\mathrm{z}}    \newcommand{\Zr}{\mathrm{Z}}  

% ================= NORMS ===========================
\newcommand{\mynorm}[2]{\| {#1} \|_{#2}}
%\newcommand{\norm}[2]{\mynorm{#1}{#2}}
\newcommand{\bignorm}[2]{\left\| {#1} \right\|_{#2}}

\newcommand{\onenorm}[1]{\mynorm{#1}{1}}
\newcommand{\bigonenorm}[1]{\bignorm{#1}{1}}

\newcommand{\infnorm}[1]{\mynorm{#1}{\infty}}
\newcommand{\biginfnorm}[1]{\bignorm{#1}{\infty}}

\newcommand{\oneinf}{\ell_{1,\infty}}
\newcommand{\onetwo}{\ell_{1,2}}
\newcommand{\oneinfnorm}[1]{\mynorm{#1}{1,\infty}}
\newcommand{\bigoneinfnorm}[1]{\bignorm{#1}{1,\infty}}

\newcommand{\onetwonorm}[1]{\mynorm{#1}{1,2}}
\newcommand{\bigonetwonorm}[1]{\bignorm{#1}{1,2}}

\newcommand{\twonorm}[1]{\mynorm{#1}{2}}
\newcommand{\bigtwonorm}[1]{\bignorm{#1}{2}}

\newcommand{\znorm}[1]{\mynorm{#1}{0}}
\newcommand{\bigznorm}[1]{\bignorm{#1}{0}}

\newcommand{\frob}[1]{\|{#1}\|_{\text{F}}}
\newcommand{\bigfrob}[1]{\bignorm{#1}{\text{F}}}


% ================ SUMs, INTEGRALS, WITHOUT LIMITS ================
\newcommand{\nlsum}{\sum\nolimits}
\newcommand{\nlprod}{\prod\nolimits}
\newcommand{\nlint}{\int\nolimits}
\newcommand{\nlmin}{\min\nolimits}


% =============== USEFUL SETS, FIELDS, ETC. ===========================
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\matbb{C}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\posdef}[1]{S_{++}^{#1}}
\newcommand{\semidef}[1]{S_+^{#1}}

% =============== MISC CONSTANTS ============================
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}
\newcommand{\fourth}{\tfrac{1}{4}}
\newcommand{\onehalf}{\tfrac{3}{2}}


% %%%%%%%%%%% MATH KEYWORDS %%%%%%%%%%%%%%%%%%%%%%%%%%
%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator{\dom}{dom}
%\DeclareMathOperator{\interior}{int}
%\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\ri}{ri}
%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\trace}{Tr}
%\DeclareMathOperator{\Diag}{Diag}
%\DeclareMathOperator{\range}{range}
%\DeclareMathOperator{\vect}{vec}
%\DeclareMathOperator{\prox}{prox}
%\DeclareMathOperator{\intr}{int}
%\DeclareMathOperator{\relint}{ri}

%\let\proof\relax
%\let\endproof\relax
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{example}{Example}
%\newtheorem{proposition}[theorem]
%\newtheorem{corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}


% SS: 6th June, 2011 --- I have upper-cased everything to match the style used
% in the book; lower case references are not to be used in the book; if they
% are, those are the typos!

% === References to figures, theorems, etc. ===
\newcommand{\prop}[1]{Proposition~\protect\ref{#1}}
\newcommand{\coro}[1]{Corollary~\protect\ref{#1}}
\newcommand{\rema}[1]{Remark~\protect\ref{#1}}
\newcommand{\exam}[1]{Example~\protect\ref{#1}}
\newcommand{\appl}[1]{Application~\protect\ref{#1}}
\newcommand{\opti}[1]{Optimization Problem~\protect\ref{#1}}
\newcommand{\defi}[1]{Definition~\protect\ref{#1}}
%\newcommand{\prob}[1]{Problem~\protect\ref{#1}}
% [SN]: lowercase \theo, uppercase \Theo
\newcommand{\Theo}[1]{Theorem~\protect\ref{#1}}
\newcommand{\theo}[1]{Theorem~\protect\ref{#1}}
% [SN]: lowercase \fig, uppcase \Fig
\newcommand{\Fig}[1]{Figure~\protect\ref{#1}}
\newcommand{\fig}[1]{Figure~\protect\ref{#1}}
\newcommand{\tab}[1]{Table~\protect\ref{#1}}
\newcommand{\chap}[1]{Chapter~\protect\ref{#1}}
% [SN]: lowercase \sec, uppcase \Sec
\newcommand{\Sec}[1]{Section~\protect\ref{#1}}
\renewcommand{\sec}[1]{Section~\protect\ref{#1}} % SS: but why?????? it shd always be uppercase!
\newcommand{\app}[1]{Appendix~\protect\ref{#1}}
\newcommand{\eq}[1]{(\protect\ref{#1})}
\newcommand{\pag}[1]{page \protect\pageref{#1}}

% === Marginal notes ===
% To use marginal notes, type in \margin{this goes into the margin}
\newcommand{\margin}[1]{\marginpar[\flushleft{#1}]{right}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%=========Special Functions======
\newcommand{\indicator}[1]{$\mathbbm{1}$\big[#1\big]}

\def\abovestrut#1{\rule[0in]{0in}{#1}\ignorespaces}
\def\belowstrut#1{\rule[-#1]{0in}{#1}\ignorespaces}

\def\abovespace{\abovestrut{0.20in}}
\def\aroundspace{\abovestrut{0.20in}\belowstrut{0.10in}}
\def\belowspace{\belowstrut{0.10in}}
\newtheorem{corollary}[theorem]{Corollary}

\newcommand{\NN}{Z}
\newcommand{\NNT}{Z_{\bf{\theta}}}



==> arxiv copy/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
% basic notation
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Nats}{\mathbb{N}}
\newcommand{\indic}[1]{\mathbbm{1}_{#1}}

%\renewcommand{\expect}[2]{\mathop{\mathbb{E}}\limits_{#1}\big[#2\big]\!\!}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\covnump}[1]{{\cal C}_p(\calX, #1)}
\newcommand{\coveps}{\gamma}



\newcommand{\wid}{k}
\newcommand{\Din}{d_{in}}
\newcommand{\Dout}{d_{out}}
\newcommand{\ReDout}{\Re^{\Dout}}
\newcommand{\bx}{x}%\xvector{x}}
\newcommand{\by}{y}
\newcommand{\bxprime}{\tilde{x}}%\xvector{\tilde{x}}}
\newcommand{\bW}{W}%\xvector{W}}
\newcommand{\bias}{b}
\newcommand{\uU}{U\xfunction}%\xvectorfun{u}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bones}{\boldsymbol{1}}
\newcommand{\conv}{\ast}

\newcommand{\row}[1]{_{#1,.}}
\newcommand{\cell}[2]{_{#1,#2}}
\newcommand{\elem}[1]{_{#1}}
\newcommand{\inv}{^{-1}}

%%%%%%%%
% notation for computation graph
%%%%%%%%

\newcommand{\normt}[1]{\norm{#1}_2}
\newcommand{\norminf}[1]{\norm{#1}_{\infty}}
\newcommand{\normp}[1]{\norm{#1}_p}
\newcommand{\network}{g}
\newcommand{\cnet}{\hat{g}\xfunction}

\newcommand{\lipp}{\Lambda_p}
\newcommand{\liplossp}{\lambda_p}
\newcommand{\liplosst}{\lambda_2}
\newcommand{\liplossinf}{\lambda_\infty}

\newcommand{\lipgp}{\Lambda_p}
\newcommand{\lipgt}{\Lambda_2}
\newcommand{\lipginf}{\Lambda_{\infty}}

\newcommand{\bdc}{z}

\newcommand{\graph}{G}
\newcommand{\nodes}{{\cal N}}
\newcommand{\edges}{{\cal E}}
\newcommand{\nod}{n}
\newcommand{\nodind}[1]{^{(#1)}}
\newcommand{\layerfunc}{\phi}

\newcommand{\loss}{\ell}
\newcommand{\logsoftmax}{\ell}
\newcommand{\Loss}{L\xfunction}
\newcommand{\Lossadv}[3]{L_{adv}(#1, #2, #3)}


\newcommand{\child}{{\tt c}}
\newcommand{\childind}[1]{^{#1}}
\newcommand{\layer}{\phi}
\newcommand{\resc}{R}
\newcommand{\self}{{\tt self}}
\newcommand{\gradinpar}{g_{par}}
\newcommand{\gradweight}{g_{wei}}
\newcommand{\gradbias}{g_{bia}}
\newcommand{\gradin}{g_{in}}

\newcommand{\xin}{x}
\newcommand{\xout}{\hat{x}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% general notation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Dx}{\Re^D}
%\newcommand{\Dc}{\Re^{\nC}}
\newcommand{\Cset}{{\cal Y}}
\newcommand{\params}{W}
\newcommand{\Dparams}{{\cal W}}
\newcommand{\paramsk}{W\childind{k}}
\newcommand{\ccc}{{\bar{y}}}
\newcommand{\nC}{Y}

\newcommand{\intint}[1]{[[#1]]}
\newcommand{\inint}[1]{\in\intint{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% the adversary
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\adv}[1]{\tilde{#1}}
\newcommand{\perturb}[1]{\delta_{#1}}
\newcommand{\adveps}{\epsilon}


==> definitions.tex <==
\usepackage{graphicx} % more modern
%\usepackage{epsfig} % less modern
%\usepackage[round,authoryear,sort]{natbib}
\usepackage{amsmath,amsthm,amssymb,bbm,stmaryrd,bm}
%\usepackage{url}

\usepackage{dsfont}
\usepackage{color}
\usepackage{wrapfig}
\usepackage{listing}
\usepackage{amsopn}
%\usepackage[breaklinks=true]{hyperref}

\newcommand{\todo}[1]{{\color{red}{To do: #1}}}

% %%%%%%%%%%%%%  VECTORS %%%%%%%%%%%%%%%%%%%
\newcommand{\bmt}[1]{\bm{#1}^T} % transpose of a vector
% INNER PRODUCT <x,y>
\newcommand{\ip}[2]{\langle {#1},\, {#2} x`\rangle}

% \va, \vb etc. type bold letters; notice exception at \vech -- coz. \vh is a
% predefined thing in latex; 
% additional commands include \vah -- read as vector a hat, 
% or \ah -- a hat and so on
\newcommand{\va}{\bm{a}}       \newcommand{\vah}{\hat{\bm{a}}}        \newcommand{\ah}{\hat{a}}
\newcommand{\vb}{\bm{b}}       \newcommand{\vbh}{\hat{\bm{b}}}        \newcommand{\bh}{\hat{b}}
\newcommand{\vc}{\bm{c}}       \newcommand{\vch}{\hat{\bm{c}}}        \newcommand{\ch}{\hat{c}}
\newcommand{\vd}{\bm{d}}       \newcommand{\vdh}{\hat{\bm{d}}}        \newcommand{\dhat}{\hat{d}}
\newcommand{\ve}{\bm{e}}       \newcommand{\veh}{\hat{\bm{e}}}        \newcommand{\eh}{\hat{e}}
\newcommand{\vf}{\bm{f}}       \newcommand{\vfh}{\hat{\bm{f}}}        \newcommand{\fh}{\hat{f}}
\newcommand{\vg}{\bm{g}}       \newcommand{\vgh}{\hat{\bm{g}}}        \newcommand{\gh}{\hat{g}}
\newcommand{\vech}{\bm{h}}     \newcommand{\vhh}{\hat{\bm{h}}}        \newcommand{\hh}{\hat{h}}
\newcommand{\vi}{\bm{i}}       \newcommand{\vih}{\hat{\bm{i}}}        \newcommand{\ih}{\hat{i}}
\newcommand{\vj}{\bm{j}}       \newcommand{\vjh}{\hat{\bm{j}}}        \newcommand{\jh}{\hat{j}}
\newcommand{\vk}{\bm{k}}       \newcommand{\vkh}{\hat{\bm{k}}}        \newcommand{\kh}{\hat{k}}
\newcommand{\vl}{\bm{l}}       \newcommand{\vlh}{\hat{\bm{l}}}        \newcommand{\lh}{\hat{l}}
\newcommand{\vm}{\bm{m}}       \newcommand{\vmh}{\hat{\bm{m}}}        \newcommand{\mh}{\hat{m}}
\newcommand{\vn}{\bm{n}}       \newcommand{\vnh}{\hat{\bm{n}}}        \newcommand{\nh}{\hat{n}}
\newcommand{\vo}{\bm{o}}       \newcommand{\voh}{\hat{\bm{o}}}        \newcommand{\oh}{\hat{o}}
\newcommand{\vp}{\bm{p}}       \newcommand{\vph}{\hat{\bm{p}}}        \newcommand{\ph}{\hat{p}}
\newcommand{\vq}{\bm{q}}       \newcommand{\vqh}{\hat{\bm{q}}}        \newcommand{\qh}{\hat{q}}
\newcommand{\vr}{\bm{r}}       \newcommand{\vrh}{\hat{\bm{r}}}        \newcommand{\rh}{\hat{r}}
\newcommand{\vs}{\bm{s}}       \newcommand{\vsh}{\hat{\bm{s}}}        \newcommand{\sh}{\hat{s}}
\newcommand{\vt}{\bm{t}}       \newcommand{\vth}{\hat{\bm{t}}}        \newcommand{\that}{\hat{t}}
\newcommand{\vu}{\bm{u}}       \newcommand{\vuh}{\hat{\bm{u}}}        \newcommand{\uh}{\hat{u}}
\newcommand{\vv}{\bm{v}}       \newcommand{\vvh}{\hat{\bm{v}}}        \newcommand{\vh}{\hat{v}}
\newcommand{\vw}{\bm{w}}       \newcommand{\vwh}{\hat{\bm{w}}}        \newcommand{\wh}{\hat{w}}
\newcommand{\vx}{\bm{x}}       \newcommand{\vxh}{\hat{\bm{x}}}        \newcommand{\xh}{\hat{x}}
\newcommand{\vy}{\bm{y}}       \newcommand{\vyh}{\hat{\bm{y}}}        \newcommand{\yh}{\hat{y}}
\newcommand{\vz}{\bm{z}}       \newcommand{\vzh}{\hat{\bm{z}}}        \newcommand{\zh}{\hat{z}}

% %%%%%%%%%%%%%%%%%%%% BOLD GREEK %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Same convention as for ordinary roman letters above
\newcommand{\valpha}  {\bm{\alpha}}      \newcommand{\valphah}  {\hat{\bm{\alpha}}}   
\newcommand{\vbeta}   {\bm{\beta}}       \newcommand{\vbetah}   {\hat{\bm{\beta}}}    
\newcommand{\vdelta}  {\bm{\delta}}      \newcommand{\vdeltah}  {\hat{\bm{\delta}}}   
\newcommand{\vepsilon}{\bm{\epsilon}}    \newcommand{\vepsilonh}{\hat{\bm{\epsilon}}} 
\newcommand{\vphi}    {\bm{\phi}}        \newcommand{\vphih}    {\hat{\bm{\phi}}}     
\newcommand{\vgamma}  {\bm{\gamma}}      \newcommand{\vgammah}  {\hat{\bm{\gamma}}}   
\newcommand{\veta}    {\bm{\eta}}        \newcommand{\vetah}    {\hat{\bm{\eta}}}     
\newcommand{\vtheta}  {\bm{\theta}}      \newcommand{\vthetah}  {\hat{\bm{\theta}}}   
\newcommand{\vkappa}  {\bm{\kappa}}      \newcommand{\vkappah}  {\hat{\bm{\kappa}}}   
\newcommand{\vlambda} {\bm{\lambda}}     \newcommand{\vlambdah} {\hat{\bm{\lambda}}}  
\newcommand{\vmu}     {\bm{\mu}}         \newcommand{\vmuh}     {\hat{\bm{\mu}}}      
\newcommand{\vnu}     {\bm{\nu}}         \newcommand{\vnuh}     {\hat{\bm{\nu}}}      
\newcommand{\vpi}     {\bm{\pi}}         \newcommand{\vpih}     {\hat{\bm{\pi}}}      
\newcommand{\vchi}    {\bm{\chi}}        \newcommand{\vchih}    {\hat{\bm{\chi}}}     
\newcommand{\vrho}    {\bm{\rho}}        \newcommand{\vrhoh}    {\hat{\bm{\rho}}}     
\newcommand{\vsigma}  {\bm{\sigma}}      \newcommand{\vsigmah}  {\hat{\bm{\sigma}}}   
\newcommand{\vtau}    {\bm{\tau}}        \newcommand{\vtauh}    {\hat{\bm{\tau}}}     
\newcommand{\vupsilon}{\bm{\upsilon}}    \newcommand{\vupsilonh}{\hat{\bm{\upsilon}}} 
\newcommand{\vomega}  {\bm{\omega}}      \newcommand{\vomegah}  {\hat{\bm{\omega}}}   
\newcommand{\vxi}     {\bm{\xi}}         \newcommand{\vxih}     {\hat{\bm{\xi}}}      
\newcommand{\vpsi}    {\bm{\psi}}        \newcommand{\vpsih}    {\hat{\bm{\psi}}}     
\newcommand{\vzeta}   {\bm{\zeta}}       \newcommand{\vzetah}   {\hat{\bm{\zeta}}}

% %%%%%%%%%%%%%  MATRICES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\newcommand{\ma}{\bm{A}}       \newcommand{\mah}{\hat{\bm{A}}}   
\newcommand{\mb}{\bm{B}}       \newcommand{\mbh}{\hat{\bm{B}}}   
\newcommand{\mc}{\bm{C}}       \newcommand{\mch}{\hat{\bm{C}}}   
\newcommand{\md}{\bm{D}}       \newcommand{\mdh}{\hat{\bm{D}}}   
\newcommand{\me}{\bm{E}}       \newcommand{\meh}{\hat{\bm{E}}}   
\newcommand{\mf}{\bm{F}}       \newcommand{\mfh}{\hat{\bm{F}}}   
\newcommand{\mg}{\bm{G}}       \newcommand{\mgh}{\hat{\bm{G}}}   
\newcommand{\mH}{\bm{H}}       \newcommand{\mhh}{\hat{\bm{H}}}   
\newcommand{\mi}{\bm{I}}       \newcommand{\mih}{\hat{\bm{I}}}   
\newcommand{\mj}{\bm{J}}       \newcommand{\mjh}{\hat{\bm{J}}}   
\newcommand{\mk}{\bm{K}}       \newcommand{\mkh}{\hat{\bm{K}}}   
\newcommand{\ml}{\bm{L}}       \newcommand{\mlh}{\hat{\bm{L}}}   
\newcommand{\mm}{\bm{M}}       \newcommand{\mmh}{\hat{\bm{M}}}   
\newcommand{\mn}{\bm{N}}       \newcommand{\mnh}{\hat{\bm{N}}}   
\newcommand{\mo}{\bm{O}}       \newcommand{\moh}{\hat{\bm{O}}}   
\newcommand{\mP}{\bm{P}}       \newcommand{\mph}{\hat{\bm{P}}}   
\newcommand{\mq}{\bm{Q}}       \newcommand{\mqh}{\hat{\bm{Q}}}   
\newcommand{\mr}{\bm{R}}       \newcommand{\mrh}{\hat{\bm{R}}}   
\newcommand{\ms}{\bm{S}}       \newcommand{\msh}{\hat{\bm{S}}}   
\newcommand{\mT}{\bm{T}}       \newcommand{\mth}{\hat{\bm{T}}}   
\newcommand{\mU}{\bm{U}}       \newcommand{\muh}{\hat{\bm{U}}}   
\newcommand{\mv}{\bm{V}}       \newcommand{\mvh}{\hat{\bm{V}}}   
\newcommand{\mw}{\bm{W}}       \newcommand{\mwh}{\hat{\bm{W}}}   
\newcommand{\mx}{\bm{X}}       \newcommand{\mxh}{\hat{\bm{X}}}   
\newcommand{\my}{\bm{Y}}       \newcommand{\myh}{\hat{\bm{Y}}}   
\newcommand{\mz}{\bm{Z}}       \newcommand{\mzh}{\hat{\bm{Z}}}   

%%%%%%%%%%%%%%%%%%%%%%%%% CALLIGRAPHIC LETTERS %%%%%%%%%%%%%%%%%%%%%
\newcommand{\ac}{\mathcal{a}}    \newcommand{\Ac}{\mathcal{A}}  
\newcommand{\bc}{\mathcal{b}}    \newcommand{\Bc}{\mathcal{B}}  
\newcommand{\cc}{\mathcal{c}}    \newcommand{\Cc}{\mathcal{C}}  
\newcommand{\dc}{\mathcal{d}}    \newcommand{\Dc}{\mathcal{D}}  
\newcommand{\ec}{\mathcal{e}}    \newcommand{\Ec}{\mathcal{E}}  
\newcommand{\fc}{\mathcal{f}}    \newcommand{\Fc}{\mathcal{F}}  
\newcommand{\gc}{\mathcal{g}}    \newcommand{\Gc}{\mathcal{G}}  
\newcommand{\hc}{\mathcal{h}}    \newcommand{\Hc}{\mathcal{H}}  
\newcommand{\ic}{\mathcal{i}}    \newcommand{\Ic}{\mathcal{I}}  
\newcommand{\jc}{\mathcal{j}}    \newcommand{\Jc}{\mathcal{J}}  
\newcommand{\kc}{\mathcal{k}}    \newcommand{\Kc}{\mathcal{K}}  
\newcommand{\lc}{\mathcal{l}}    \newcommand{\Lc}{\mathcal{L}}  
\newcommand{\mcal}{\mathcal{m}}  \newcommand{\Mc}{\mathcal{M}}  
\newcommand{\nc}{\mathcal{n}}    \newcommand{\Nc}{\mathcal{N}}  
\newcommand{\oc}{\mathcal{o}}    \newcommand{\Oc}{\mathcal{O}}  
\newcommand{\pc}{\mathcal{p}}    \newcommand{\Pc}{\mathcal{P}}  
\newcommand{\qc}{\mathcal{q}}    \newcommand{\Qc}{\mathcal{Q}}  
\newcommand{\rc}{\mathcal{r}}    \newcommand{\Rc}{\mathcal{R}}  
\newcommand{\scal}{\mathcal{s}}  \newcommand{\Sc}{\mathcal{S}}  
\newcommand{\tc}{\mathcal{t}}    \newcommand{\Tc}{\mathcal{T}}  
\newcommand{\uc}{\mathcal{u}}    \newcommand{\Uc}{\mathcal{U}}  
\newcommand{\vcal}{\mathcal{v}}  \newcommand{\Vc}{\mathcal{V}}  
\newcommand{\wc}{\mathcal{w}}    \newcommand{\Wc}{\mathcal{W}}  
\newcommand{\xc}{\mathcal{x}}    \newcommand{\Xc}{\mathcal{X}}  
\newcommand{\yc}{\mathcal{y}}    \newcommand{\Yc}{\mathcal{Y}}  
\newcommand{\zc}{\mathcal{z}}    \newcommand{\Zc}{\mathcal{Z}}  

%%%%%%%%%%%%%%%%%%%%%%%%% MATHEMATIC LETTERS %%%%%%%%%%%%%%%%%%%%%
\newcommand{\ar}{\mathrm{a}}    \newcommand{\Ars}{\mathrm{A}}  
\newcommand{\br}{\mathrm{b}}    \newcommand{\Br}{\mathrm{B}}  
\newcommand{\crm}{\mathrm{c}}    \newcommand{\Cr}{\mathrm{C}}  
\newcommand{\dr}{\mathrm{d}}    \newcommand{\Dr}{\mathrm{D}}  
\newcommand{\er}{\mathrm{e}}    \newcommand{\Er}{\mathrm{E}}  
\newcommand{\fr}{\mathrm{f}}    \newcommand{\Fr}{\mathrm{F}}  
\newcommand{\gr}{\mathrm{g}}    \newcommand{\Gr}{\mathrm{G}}  
\newcommand{\hr}{\mathrm{h}}    \newcommand{\Hr}{\mathrm{H}}  
\newcommand{\ir}{\mathrm{i}}    \newcommand{\Ir}{\mathrm{I}}  
\newcommand{\jr}{\mathrm{j}}    \newcommand{\Jr}{\mathrm{J}}  
\newcommand{\kr}{\mathrm{k}}    \newcommand{\Kr}{\mathrm{K}}  
\newcommand{\lr}{\mathrm{l}}    \newcommand{\Lr}{\mathrm{L}}  
\newcommand{\mrml}{\mathrm{m}}  \newcommand{\Mr}{\mathrm{M}}  
\newcommand{\nr}{\mathrm{n}}    \newcommand{\Nr}{\mathrm{N}}  
\newcommand{\orm}{\mathrm{o}}    \newcommand{\Orm}{\mathrm{O}}  
\newcommand{\pr}{\mathrm{p}}    \newcommand{\Prm}{\mathrm{P}}  
\newcommand{\qr}{\mathrm{q}}    \newcommand{\Qr}{\mathrm{Q}}  
\newcommand{\rr}{\mathrm{r}}    \newcommand{\Rr}{\mathrm{R}}  
\newcommand{\srm}{\mathrm{s}}  \newcommand{\Sr}{\mathrm{S}}  
\newcommand{\tr}{\mathrm{t}}    \newcommand{\Tr}{\mathrm{T}}  
\newcommand{\ur}{\mathrm{u}}    \newcommand{\Ur}{\mathrm{U}}  
\newcommand{\vrm}{\mathrm{v}}  \newcommand{\Vr}{\mathrm{V}}  
\newcommand{\wrm}{\mathrm{w}}    \newcommand{\Wr}{\mathrm{W}}  
\newcommand{\xr}{\mathrm{x}}    \newcommand{\Xr}{\mathrm{X}}  
\newcommand{\yr}{\mathrm{y}}    \newcommand{\Yr}{\mathrm{Y}}  
\newcommand{\zr}{\mathrm{z}}    \newcommand{\Zr}{\mathrm{Z}}  

% ================= NORMS ===========================
\newcommand{\mynorm}[2]{\| {#1} \|_{#2}}
%\newcommand{\norm}[2]{\mynorm{#1}{#2}}
\newcommand{\bignorm}[2]{\left\| {#1} \right\|_{#2}}

\newcommand{\onenorm}[1]{\mynorm{#1}{1}}
\newcommand{\bigonenorm}[1]{\bignorm{#1}{1}}

\newcommand{\infnorm}[1]{\mynorm{#1}{\infty}}
\newcommand{\biginfnorm}[1]{\bignorm{#1}{\infty}}

\newcommand{\oneinf}{\ell_{1,\infty}}
\newcommand{\onetwo}{\ell_{1,2}}
\newcommand{\oneinfnorm}[1]{\mynorm{#1}{1,\infty}}
\newcommand{\bigoneinfnorm}[1]{\bignorm{#1}{1,\infty}}

\newcommand{\onetwonorm}[1]{\mynorm{#1}{1,2}}
\newcommand{\bigonetwonorm}[1]{\bignorm{#1}{1,2}}

\newcommand{\twonorm}[1]{\mynorm{#1}{2}}
\newcommand{\bigtwonorm}[1]{\bignorm{#1}{2}}

\newcommand{\znorm}[1]{\mynorm{#1}{0}}
\newcommand{\bigznorm}[1]{\bignorm{#1}{0}}

\newcommand{\frob}[1]{\|{#1}\|_{\text{F}}}
\newcommand{\bigfrob}[1]{\bignorm{#1}{\text{F}}}


% ================ SUMs, INTEGRALS, WITHOUT LIMITS ================
\newcommand{\nlsum}{\sum\nolimits}
\newcommand{\nlprod}{\prod\nolimits}
\newcommand{\nlint}{\int\nolimits}
\newcommand{\nlmin}{\min\nolimits}


% =============== USEFUL SETS, FIELDS, ETC. ===========================
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\matbb{C}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\posdef}[1]{S_{++}^{#1}}
\newcommand{\semidef}[1]{S_+^{#1}}

% =============== MISC CONSTANTS ============================
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}
\newcommand{\fourth}{\tfrac{1}{4}}
\newcommand{\onehalf}{\tfrac{3}{2}}


% %%%%%%%%%%% MATH KEYWORDS %%%%%%%%%%%%%%%%%%%%%%%%%%
%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator{\dom}{dom}
%\DeclareMathOperator{\interior}{int}
%\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\ri}{ri}
%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\trace}{Tr}
%\DeclareMathOperator{\Diag}{Diag}
%\DeclareMathOperator{\range}{range}
%\DeclareMathOperator{\vect}{vec}
%\DeclareMathOperator{\prox}{prox}
%\DeclareMathOperator{\intr}{int}
%\DeclareMathOperator{\relint}{ri}

%\let\proof\relax
%\let\endproof\relax
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{example}{Example}
%\newtheorem{proposition}[theorem]
%\newtheorem{corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}


% SS: 6th June, 2011 --- I have upper-cased everything to match the style used
% in the book; lower case references are not to be used in the book; if they
% are, those are the typos!

% === References to figures, theorems, etc. ===
\newcommand{\prop}[1]{Proposition~\protect\ref{#1}}
\newcommand{\coro}[1]{Corollary~\protect\ref{#1}}
\newcommand{\rema}[1]{Remark~\protect\ref{#1}}
\newcommand{\exam}[1]{Example~\protect\ref{#1}}
\newcommand{\appl}[1]{Application~\protect\ref{#1}}
\newcommand{\opti}[1]{Optimization Problem~\protect\ref{#1}}
\newcommand{\defi}[1]{Definition~\protect\ref{#1}}
%\newcommand{\prob}[1]{Problem~\protect\ref{#1}}
% [SN]: lowercase \theo, uppercase \Theo
\newcommand{\Theo}[1]{Theorem~\protect\ref{#1}}
\newcommand{\theo}[1]{Theorem~\protect\ref{#1}}
% [SN]: lowercase \fig, uppcase \Fig
\newcommand{\Fig}[1]{Figure~\protect\ref{#1}}
\newcommand{\fig}[1]{Figure~\protect\ref{#1}}
\newcommand{\tab}[1]{Table~\protect\ref{#1}}
\newcommand{\chap}[1]{Chapter~\protect\ref{#1}}
% [SN]: lowercase \sec, uppcase \Sec
\newcommand{\Sec}[1]{Section~\protect\ref{#1}}
\renewcommand{\sec}[1]{Section~\protect\ref{#1}} % SS: but why?????? it shd always be uppercase!
\newcommand{\app}[1]{Appendix~\protect\ref{#1}}
\newcommand{\eq}[1]{(\protect\ref{#1})}
\newcommand{\pag}[1]{page \protect\pageref{#1}}

% === Marginal notes ===
% To use marginal notes, type in \margin{this goes into the margin}
\newcommand{\margin}[1]{\marginpar[\flushleft{#1}]{right}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%=========Special Functions======
\newcommand{\indicator}[1]{$\mathbbm{1}$\big[#1\big]}

\def\abovestrut#1{\rule[0in]{0in}{#1}\ignorespaces}
\def\belowstrut#1{\rule[-#1]{0in}{#1}\ignorespaces}

\def\abovespace{\abovestrut{0.20in}}
\def\aroundspace{\abovestrut{0.20in}\belowstrut{0.10in}}
\def\belowspace{\belowstrut{0.10in}}
\newtheorem{corollary}[theorem]{Corollary}

\newcommand{\NN}{Z}
\newcommand{\NNT}{Z_{\bf{\theta}}}


